Convective core sizes in rotating massive stars: I. Constraints from solar metallicity OB field stars

Spectroscopic studies of Galactic O and B stars show that many stars with masses above 8 M$_{\odot}$ are observed in the HR diagram just beyond the Main-Sequence (MS) band predicted by stellar models computed with a moderate overshooting. This may be an indication that the convective core sizes in stars in the upper part of the HR diagram are larger than predicted by these models. Combining stellar evolution models and spectroscopic parameters derived for a large sample of Galactic O and B stars, including brand new information about their projected rotational velocities, we reexamine the question of the convective core size in MS massive stars. We confirm that for stars more massive than about 8 M$_{\odot}$, the convective core size at the end of the MS phase increases more rapidly with the mass than in models computed with a constant step overshoot chosen to reproduce the main sequence width in the low mass range (around 2 M$_{\odot}$). This conclusion is valid for both the cases of non-rotating models and rotating models either with a moderate or a strong angular momentum transport. The increase of the convective core mass with the mass obtained from the TAMS position is, however, larger than the one deduced from the surface velocity drop for masses above about 15 M$_{\odot}$. Although observations available at the moment cannot decide what is the best choice between the core sizes given by the TAMS and the velocity drop, we discuss different methods to get out of this dilemma. At the moment, comparisons with eclipsing binaries seem to favor the solution given by the velocity drop. While we confirm the need for larger convective cores at higher masses, we find tensions in-between different methods for stars more massive than 15 M$_{\odot}$. The use of single-aged stellar populations (non-interacting binaries or stellar clusters) would be a great asset to resolve this tension.

==> Figures/table.tex <==
\begin{longtable*}{lrrrrrrrrrrrr}
\toprule
 Mass &  VVc &  Mag &  Overshoot &         tau\_H &        tau\_He &      tau\_cross &    sL\_max &    He\_core &  Vsurf\_end\_MS &  NHrel\_end\_MS &  Omega\_s\_cen &  Ltot\_Lini \\
\midrule
\endhead
\midrule
\multicolumn{13}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
  7.0 &  0.0 &  0.0 &        0.1 &  4.306201e+07 &  7.291204e+06 &  373809.631509 &  2.765435 &   0.000000 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  7.0 &  0.0 &  0.0 &        0.2 &  4.634582e+07 &  5.606260e+06 &  211676.658146 &  2.805896 &   0.000000 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  7.0 &  0.0 &  0.0 &        0.3 &  5.000281e+07 &  4.426482e+06 &  128608.804256 &  2.851113 &   0.000000 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  7.0 &  0.0 &  0.0 &        0.4 &  5.306942e+07 &  3.874869e+06 &   83864.917190 &  2.908913 &   0.000000 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  7.0 &  0.0 &  0.0 &        0.5 &  5.635157e+07 &  3.463132e+06 &   55071.376908 &  2.969514 &   0.086077 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  7.0 &  0.0 &  0.0 &        0.6 &  5.983829e+07 &           NaN &   40073.569493 &  3.031541 &   0.708146 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  7.0 &  0.2 &  0.0 &        0.1 &  4.918455e+07 &  6.654175e+06 &  340633.026746 &  2.849817 &   0.000000 &         82.30 &  3.960930e-02 &     0.189678 &   0.998200 \\
  7.0 &  0.2 &  0.0 &        0.2 &  5.279322e+07 &  4.998036e+06 &  185721.256614 &  2.915154 &   0.000000 &         84.90 &  4.853780e-02 &     0.193617 &   0.997113 \\
  7.0 &  0.2 &  0.0 &        0.3 &  5.746981e+07 &  3.856244e+06 &  100595.029121 &  2.981495 &   0.124563 &         86.70 &  5.988742e-02 &     0.190326 &   0.995246 \\
  7.0 &  0.2 &  0.0 &        0.4 &  6.038784e+07 &  3.298104e+06 &   62529.261268 &  3.045104 &   0.061574 &         88.80 &  7.081680e-02 &     0.181052 &   0.992384 \\
  7.0 &  0.2 &  0.0 &        0.5 &  6.407241e+07 &  2.865340e+06 &   42440.490118 &  3.114487 &   0.693977 &         91.60 &  8.148859e-02 &     0.177929 &   0.987555 \\
  7.0 &  0.2 &  0.0 &        0.6 &  6.769745e+07 &  2.538811e+06 &   30137.990807 &  3.187531 &   1.221841 &         94.90 &  9.627288e-02 &     0.174497 &   0.979694 \\
  7.0 &  0.2 &  1.0 &        0.1 &  4.867080e+07 &  6.314766e+06 &  342760.696504 &  2.849351 &   0.000000 &         82.20 &  3.918186e-02 &     0.190330 &   0.998223 \\
  7.0 &  0.2 &  1.0 &        0.2 &  5.277829e+07 &  4.939549e+06 &  186966.096867 &  2.914951 &   0.000000 &         84.80 &  4.841581e-02 &     0.194660 &   0.997120 \\
  7.0 &  0.2 &  1.0 &        0.3 &  5.674878e+07 &  4.490929e+06 &  101303.656056 &  2.980339 &   0.125263 &         87.00 &  5.872028e-02 &     0.190280 &   0.995314 \\
  7.0 &  0.2 &  1.0 &        0.4 &  6.038033e+07 &  3.305675e+06 &   63243.216581 &  3.044555 &   0.337257 &         88.90 &  6.978274e-02 &     0.186474 &   0.992417 \\
  7.0 &  0.2 &  1.0 &        0.5 &  6.407241e+07 &  2.865340e+06 &   42440.490118 &  3.114487 &   0.693977 &         91.60 &  8.148859e-02 &     0.177929 &   0.987555 \\
  7.0 &  0.2 &  1.0 &        0.6 &  6.769745e+07 &  2.538811e+06 &   30137.990807 &  3.187531 &   1.221841 &         94.90 &  9.627288e-02 &     0.174497 &   0.979694 \\
  7.0 &  0.4 &  0.0 &        0.1 &  5.156579e+07 &  6.387866e+06 &  360029.679718 &  2.865491 &   0.000000 &        184.00 &  3.755082e-01 &     0.254592 &   0.997570 \\
  7.0 &  0.4 &  0.0 &        0.2 &  5.619149e+07 &           NaN &  177999.256421 &  2.946889 &   0.000000 &        195.00 &  3.675449e-01 &     0.263222 &   0.995586 \\
  7.0 &  0.4 &  0.0 &        0.3 &  6.021385e+07 &           NaN &  104489.589944 &  3.021389 &   0.040584 &        207.00 &  3.589767e-01 &     0.267940 &   0.992088 \\
  7.0 &  0.4 &  0.0 &        0.4 &  6.350299e+07 &  3.171415e+06 &   61824.111850 &  3.094218 &   0.132219 &        219.00 &  3.557149e-01 &     0.258226 &   0.985339 \\
  7.0 &  0.4 &  0.0 &        0.5 &  6.821281e+07 &           NaN &   40934.975377 &  3.166219 &   0.744092 &        236.00 &  3.550260e-01 &     0.254329 &   0.971762 \\
  7.0 &  0.4 &  0.0 &        0.6 &  7.085119e+07 &  2.232780e+06 &   29217.070403 &  3.246131 &   1.188406 &        220.00 &  3.831472e-01 &     0.228300 &   0.904696 \\
  7.0 &  0.4 &  1.0 &        0.1 &  6.204100e+07 &  5.325884e+06 &  281461.155413 &  3.026682 &   0.000000 &        252.00 &  7.715114e-01 &     0.423354 &   0.992081 \\
  7.0 &  0.4 &  1.0 &        0.2 &  6.599768e+07 &           NaN &  143500.887901 &  3.114301 &   0.000000 &        278.00 &  8.245295e-01 &     0.410493 &   0.986548 \\
  7.0 &  0.4 &  1.0 &        0.3 &  7.015476e+07 &           NaN &   74148.719682 &  3.207345 &   0.322350 &        291.00 &  8.798112e-01 &     0.387091 &   0.965007 \\
  7.0 &  0.4 &  1.0 &        0.4 &           NaN &           NaN &            NaN &  3.142391 &        NaN &           NaN &           NaN &          NaN &        NaN \\
  7.0 &  0.4 &  1.0 &        0.5 &           NaN &           NaN &            NaN &  3.221931 &        NaN &           NaN &           NaN &          NaN &        NaN \\
  7.0 &  0.4 &  1.0 &        0.6 &           NaN &           NaN &            NaN &  3.334585 &        NaN &           NaN &           NaN &          NaN &        NaN \\
  9.0 &  0.2 &  0.0 &        0.1 &  3.040735e+07 &  3.245500e+06 &  126210.605716 &  3.117000 &   0.008090 &         85.50 &  8.886399e-02 &     0.192989 &   0.985334 \\
  9.0 &  0.2 &  0.0 &        0.2 &  3.286883e+07 &  2.664859e+06 &   73515.062008 &  3.180778 &   0.294711 &         87.10 &  1.032574e-01 &     0.189333 &   0.978055 \\
  9.0 &  0.2 &  0.0 &        0.3 &  3.508506e+07 &           NaN &   46701.437555 &  3.244425 &   0.000000 &         88.10 &  1.145110e-01 &     0.171907 &   0.967874 \\
  9.0 &  0.2 &  0.0 &        0.4 &  3.720907e+07 &  1.938885e+06 &   32653.250730 &  3.309738 &   1.154083 &         86.90 &  1.377930e-01 &     0.169365 &   0.952952 \\
  9.0 &  0.2 &  0.0 &        0.5 &  3.934064e+07 &           NaN &   23952.916855 &  3.378772 &   1.591491 &         84.90 &  1.558621e-01 &     0.156849 &   0.930529 \\
  9.0 &  0.2 &  0.0 &        0.6 &  4.138186e+07 &  1.605757e+06 &   18650.574702 &  3.445286 &   1.970431 &         83.10 &  1.867854e-01 &     0.145864 &   0.900009 \\
  9.0 &  0.2 &  1.0 &        0.1 &  3.019353e+07 &  3.582672e+06 &  145147.112549 &  3.125001 &   0.000000 &        116.00 &  1.283864e-01 &     0.287528 &   0.981418 \\
  9.0 &  0.2 &  1.0 &        0.2 &  3.265915e+07 &           NaN &   83141.224699 &  3.189979 &   0.228221 &        119.00 &  1.752273e-01 &     0.269475 &   0.972702 \\
  9.0 &  0.2 &  1.0 &        0.3 &  3.497143e+07 &           NaN &   51759.786062 &  3.255608 &   0.496606 &        121.00 &  2.227226e-01 &     0.246274 &   0.960233 \\
  9.0 &  0.2 &  1.0 &        0.4 &  3.720212e+07 &           NaN &   34619.988823 &  3.321382 &   1.125325 &        122.00 &  2.728092e-01 &     0.226484 &   0.941991 \\
  9.0 &  0.2 &  1.0 &        0.5 &  3.942919e+07 &           NaN &   23686.478214 &  3.390189 &   0.000000 &        123.00 &  3.257210e-01 &     0.185448 &   0.914251 \\
  9.0 &  0.2 &  1.0 &        0.6 &  4.169325e+07 &           NaN &   17735.539948 &  3.463125 &   1.424587 &        122.00 &  3.883790e-01 &     0.172758 &   0.873857 \\
  9.0 &  0.4 &  0.0 &        0.1 &  3.167533e+07 &  3.377938e+06 &  134941.855193 &  3.129788 &   0.000000 &        190.00 &  4.688802e-01 &     0.254164 &   0.981659 \\
  9.0 &  0.4 &  0.0 &        0.2 &  3.443642e+07 &  2.830873e+06 &   77754.016286 &  3.209879 &   0.295529 &        199.00 &  4.627168e-01 &     0.259322 &   0.969528 \\
  9.0 &  0.4 &  0.0 &        0.3 &  3.690538e+07 &  2.094700e+06 &   47877.198220 &  3.286353 &   0.774574 &        203.00 &  4.601177e-01 &     0.253232 &   0.949338 \\
  9.0 &  0.4 &  0.0 &        0.4 &  3.908009e+07 &  1.870248e+06 &   32226.113042 &  3.359593 &   1.141353 &        203.00 &  4.611550e-01 &     0.235969 &   0.917368 \\
  9.0 &  0.4 &  0.0 &        0.5 &  4.120437e+07 &           NaN &   23183.463717 &  3.436154 &   1.449379 &        191.00 &  4.688082e-01 &     0.210472 &   0.862588 \\
  9.0 &  0.4 &  0.0 &        0.6 &  4.328455e+07 &           NaN &   17996.768246 &  3.512939 &   1.995918 &        188.00 &  4.982233e-01 &     0.205286 &   0.780920 \\
  9.0 &  0.4 &  1.0 &        0.1 &  3.900742e+07 &           NaN &   93337.839512 &  3.328396 &   0.000000 &        277.00 &  9.061641e-01 &     0.426311 &   0.942024 \\
  9.0 &  0.4 &  1.0 &        0.2 &  4.131067e+07 &           NaN &   55902.242257 &  3.418528 &   0.351240 &        302.00 &  9.506580e-01 &     0.419529 &   0.911489 \\
  9.0 &  0.4 &  1.0 &        0.3 &  4.364608e+07 &           NaN &   36326.970865 &  3.513029 &   1.059908 &        355.00 &  1.002851e+00 &     0.411753 &   0.865864 \\
  9.0 &  0.4 &  1.0 &        0.4 &           NaN &           NaN &            NaN &  3.508085 &        NaN &           NaN &           NaN &          NaN &        NaN \\
  9.0 &  0.4 &  1.0 &        0.5 &           NaN &           NaN &            NaN &  3.589513 &        NaN &           NaN &           NaN &          NaN &        NaN \\
  9.0 &  0.4 &  1.0 &        0.6 &           NaN &           NaN &            NaN &  3.684654 &        NaN &           NaN &           NaN &          NaN &        NaN \\
  9.0 &  0.0 &  0.0 &        0.1 &  2.626810e+07 &  3.495226e+06 &  147162.607756 &  3.024704 &   0.000000 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  9.0 &  0.0 &  0.0 &        0.2 &  2.831653e+07 &  2.959272e+06 &   87488.240124 &  3.063466 &   0.117780 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  9.0 &  0.0 &  0.0 &        0.3 &  3.019091e+07 &  2.805889e+06 &   58260.517933 &  3.115431 &   0.243591 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  9.0 &  0.0 &  0.0 &        0.4 &  3.202098e+07 &  2.311595e+06 &   41395.675315 &  3.170529 &   0.000000 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  9.0 &  0.0 &  0.0 &        0.5 &  3.393812e+07 &  2.116215e+06 &   31198.377352 &  3.225476 &   0.805754 &           NaN &  0.000000e+00 &          NaN &        NaN \\
  9.0 &  0.0 &  0.0 &        0.6 &  3.579326e+07 &  1.972979e+06 &   24694.987362 &  3.279502 &   1.601845 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 15.0 &  0.2 &  0.0 &        0.1 &  1.287919e+07 &           NaN &   32370.396285 &  3.606038 &   1.218314 &         63.20 &  3.023063e-01 &     0.122003 &   0.816234 \\
 15.0 &  0.2 &  0.0 &        0.2 &  1.375423e+07 &  1.140102e+06 &   22775.420804 &  3.657400 &   2.012049 &         57.40 &  3.403663e-01 &     0.102436 &   0.761845 \\
 15.0 &  0.2 &  0.0 &        0.3 &  1.461880e+07 &           NaN &   16200.736359 &  3.713520 &   2.815052 &         46.80 &  4.025599e-01 &     0.076926 &   0.693974 \\
 15.0 &  0.2 &  0.0 &        0.4 &  1.544241e+07 &           NaN &   12739.510144 &  3.764672 &   3.874246 &         38.60 &  4.724488e-01 &     0.061794 &   0.623719 \\
 15.0 &  0.2 &  0.0 &        0.5 &  1.611822e+07 &           NaN &   10347.767863 &  3.820243 &   4.500129 &         30.30 &  5.508899e-01 &     0.045639 &   0.556787 \\
 15.0 &  0.2 &  0.0 &        0.6 &  1.681809e+07 &           NaN &    9075.385790 &  3.879271 &   5.259027 &         19.30 &  6.268595e-01 &     0.028926 &   0.495285 \\
 15.0 &  0.2 &  1.0 &        0.1 &  1.286573e+07 &           NaN &   34687.415156 &  3.616562 &   1.114941 &        113.00 &  3.354620e-01 &     0.227385 &   0.765002 \\
 15.0 &  0.2 &  1.0 &        0.2 &  1.378394e+07 &           NaN &   24272.786764 &  3.675348 &   1.958551 &        101.00 &  3.739942e-01 &     0.178286 &   0.701000 \\
 15.0 &  0.2 &  1.0 &        0.3 &  1.468683e+07 &           NaN &   16438.311468 &  3.729339 &   2.962511 &         73.80 &  4.178553e-01 &     0.115290 &   0.630907 \\
 15.0 &  0.2 &  1.0 &        0.4 &  1.556504e+07 &           NaN &   12455.228254 &  3.784275 &   3.869310 &         51.60 &  5.162867e-01 &     0.071960 &   0.570449 \\
 15.0 &  0.2 &  1.0 &        0.5 &  1.631276e+07 &           NaN &    9948.240921 &  3.840233 &   4.663681 &         37.00 &  6.048194e-01 &     0.045459 &   0.522939 \\
 15.0 &  0.2 &  1.0 &        0.6 &           NaN &           NaN &            NaN &  3.790342 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 15.0 &  0.4 &  0.0 &        0.1 &  1.360735e+07 &           NaN &   32257.789970 &  3.644027 &   1.231555 &        140.00 &  6.189805e-01 &     0.179730 &   0.762270 \\
 15.0 &  0.4 &  0.0 &        0.2 &  1.464889e+07 &           NaN &   24590.362795 &  3.716159 &   2.309150 &        125.00 &  6.352689e-01 &     0.158943 &   0.669429 \\
 15.0 &  0.4 &  0.0 &        0.3 &  1.554759e+07 &           NaN &   16759.498058 &  3.781304 &   3.339697 &         92.90 &  6.633082e-01 &     0.121390 &   0.569261 \\
 15.0 &  0.4 &  0.0 &        0.4 &  1.637631e+07 &           NaN &   12567.642007 &  3.845523 &   4.136111 &         72.90 &  7.081304e-01 &     0.096090 &   0.471713 \\
 15.0 &  0.4 &  0.0 &        0.5 &  1.720281e+07 &           NaN &   10308.668484 &  3.912602 &   5.215082 &         56.80 &  7.753011e-01 &     0.081244 &   0.387322 \\
 15.0 &  0.4 &  0.0 &        0.6 &  1.803910e+07 &           NaN &    9175.870476 &  4.003883 &   6.099862 &         34.60 &  8.658442e-01 &     0.057692 &   0.311175 \\
 15.0 &  0.4 &  1.0 &        0.1 &  1.616221e+07 &           NaN &   26584.661040 &  3.811381 &   1.657429 &        220.00 &  1.040891e+00 &     0.331418 &   0.586133 \\
 15.0 &  0.4 &  1.0 &        0.2 &  1.695910e+07 &           NaN &   17824.711028 &  3.886055 &   3.108439 &        194.00 &  1.069945e+00 &     0.282598 &   0.500308 \\
 15.0 &  0.4 &  1.0 &        0.3 &  1.775760e+07 &           NaN &   12819.591085 &  3.960756 &   4.220459 &        144.00 &  1.105692e+00 &     0.205267 &   0.425079 \\
 15.0 &  0.4 &  1.0 &        0.4 &           NaN &           NaN &            NaN &  3.907926 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 15.0 &  0.4 &  1.0 &        0.5 &           NaN &           NaN &            NaN &  3.936667 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 15.0 &  0.4 &  1.0 &        0.6 &  2.009346e+07 &           NaN &    6509.542761 &  4.219776 &   8.115255 &         84.50 &  1.305685e+00 &     0.154651 &   0.325775 \\
 15.0 &  0.0 &  0.0 &        0.1 &  1.114793e+07 &  1.326060e+06 &   36863.731538 &  3.510675 &   1.107659 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 15.0 &  0.0 &  0.0 &        0.2 &  1.184175e+07 &  1.176970e+06 &   31327.015359 &  3.532806 &   1.785224 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 15.0 &  0.0 &  0.0 &        0.3 &  1.249555e+07 &  1.066472e+06 &   22456.693365 &  3.569227 &   2.175153 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 15.0 &  0.0 &  0.0 &        0.4 &  1.311365e+07 &  1.015078e+06 &   17160.344387 &  3.611290 &   2.741117 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 15.0 &  0.0 &  0.0 &        0.5 &  1.372668e+07 &           NaN &   14220.998470 &  3.655347 &   3.597564 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 15.0 &  0.0 &  0.0 &        0.6 &  1.434328e+07 &           NaN &   11833.077319 &  3.692889 &   4.194288 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 25.0 &  0.2 &  0.0 &        0.1 &  7.372024e+06 &           NaN &   10497.861841 &  3.973657 &   5.533738 &         33.70 &  5.641231e-01 &     0.056108 &   0.583122 \\
 25.0 &  0.2 &  0.0 &        0.2 &  7.813505e+06 &           NaN &    8202.494591 &  4.023661 &   7.064254 &         31.00 &  6.406205e-01 &     0.046562 &   0.511044 \\
 25.0 &  0.2 &  0.0 &        0.3 &  8.273799e+06 &           NaN &    6132.060364 &  4.088407 &   9.034137 &          6.68 &  7.474333e-01 &     0.008453 &   0.387430 \\
 25.0 &  0.2 &  0.0 &        0.4 &           NaN &           NaN &            NaN &  4.030767 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.2 &  0.0 &        0.5 &           NaN &           NaN &            NaN &  4.082521 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.2 &  0.0 &        0.6 &           NaN &           NaN &            NaN &  4.184734 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.2 &  1.0 &        0.1 &  7.455963e+06 &           NaN &   11229.757483 &  3.982575 &   5.430443 &         57.60 &  6.095031e-01 &     0.086656 &   0.520154 \\
 25.0 &  0.2 &  1.0 &        0.2 &  7.864626e+06 &           NaN &    8202.038426 &  4.027529 &   6.689861 &         44.20 &  6.834005e-01 &     0.053198 &   0.482488 \\
 25.0 &  0.2 &  1.0 &        0.3 &           NaN &           NaN &            NaN &  3.976706 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.2 &  1.0 &        0.4 &           NaN &           NaN &            NaN &  4.008815 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.2 &  1.0 &        0.5 &           NaN &           NaN &            NaN &  3.912154 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.2 &  1.0 &        0.6 &           NaN &           NaN &            NaN &  3.890587 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.4 &  0.0 &        0.1 &  7.937872e+06 &           NaN &   10166.883578 &  4.026950 &   6.074351 &         70.20 &  7.694909e-01 &     0.091705 &   0.437239 \\
 25.0 &  0.4 &  0.0 &        0.2 &  8.434277e+06 &           NaN &    7610.238259 &  4.090648 &   8.042664 &         41.40 &  8.615520e-01 &     0.057727 &   0.331059 \\
 25.0 &  0.4 &  0.0 &        0.3 &  8.753764e+06 &           NaN &    6332.031119 &  4.151765 &   9.766803 &         25.90 &  9.571391e-01 &     0.038148 &   0.255586 \\
 25.0 &  0.4 &  0.0 &        0.4 &  9.408271e+06 &           NaN &    2757.822307 &  4.232945 &  12.269945 &          8.33 &  1.157220e+00 &     0.018946 &   0.766768 \\
 25.0 &  0.4 &  0.0 &        0.5 &           NaN &           NaN &            NaN &  4.194313 &        NaN &           NaN &           NaN &          NaN &        NaN \\
 25.0 &  0.4 &  0.0 &        0.6 &  9.944000e+06 &           NaN &    3320.582129 &  4.305719 &  10.803718 &         13.60 &  2.319223e+00 &     0.268562 &   0.036804 \\
 25.0 &  0.4 &  1.0 &        0.1 &  8.985550e+06 &           NaN &    6580.634473 &  4.150092 &   7.723800 &         37.80 &  1.189646e+00 &     0.061873 &   0.264072 \\
 25.0 &  0.4 &  1.0 &        0.2 &  9.263107e+06 &           NaN &    8060.447830 &  4.222894 &   9.560593 &         24.20 &  1.236538e+00 &     0.038254 &   0.239571 \\
 25.0 &  0.4 &  1.0 &        0.3 &  9.581493e+06 &           NaN &    4921.490241 &  4.273773 &  11.725282 &         15.90 &  1.310873e+00 &     0.027104 &   0.210945 \\
 25.0 &  0.4 &  1.0 &        0.4 &  9.974083e+06 &           NaN &    2309.185544 &  4.336194 &  13.698485 &         15.50 &  1.523705e+00 &     0.044709 &   0.174140 \\
 25.0 &  0.4 &  1.0 &        0.5 &  1.014645e+07 &           NaN &    2526.454926 &  4.308944 &  10.798387 &         22.20 &  2.383201e+00 &     0.194737 &   0.089989 \\
 25.0 &  0.4 &  1.0 &        0.6 &  1.020481e+07 &           NaN &    4198.161035 &  4.358830 &  11.897359 &         26.20 &  2.403589e+00 &     0.235776 &   0.090781 \\
 25.0 &  0.0 &  0.0 &        0.1 &  6.269340e+06 &           NaN &   15410.268855 &  3.918948 &   4.130804 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 25.0 &  0.0 &  0.0 &        0.2 &  6.586693e+06 &           NaN &   14762.231967 &  3.924526 &   5.795393 &           NaN &  0.000000e+00 &          NaN &        NaN \\
 25.0 &  0.0 &  0.0 &        0.3 &  6.873327e+06 &           NaN &   12475.492077 &  3.934584 &   7.010943 &           NaN &  6.691131e-08 &          NaN &        NaN \\
 25.0 &  0.0 &  0.0 &        0.4 &  7.123748e+06 &           NaN &    9768.800330 &  3.952150 &   7.869957 &           NaN &  9.328181e-08 &          NaN &        NaN \\
 25.0 &  0.0 &  0.0 &        0.5 &  7.385707e+06 &           NaN &    7442.440854 &  3.977670 &   8.831244 &           NaN &  2.458972e-07 &          NaN &        NaN \\
 25.0 &  0.0 &  0.0 &        0.6 &  7.651782e+06 &           NaN &    6117.196491 &  4.008814 &   9.627384 &           NaN &  5.435503e-07 &          NaN &        NaN \\
\end{longtable*}

